A Study of Subsurface Convection Zones of Fast Rotating Massive Stars

The subsurface convective zones (CZs) of massive stars significantly influences many of their key characteristics. Previous studies have paid little attention to the impact of rotation on the subsurface convective zone (CZ), so we aim to investigate the evolution of this zone in rapidly rotating massive stars. We use the Modules for Experiments in Stellar Astrophysics (MESA) to simulate the subsurface CZs of massive stars during the main sequence phase. We establish stellar models with initial masses ranging from 5 $M_{\odot}$ to 120 $M_{\odot}$, incorporating four metallicities (Z = 0.02, 0.006, 0.002, and 0.0001) and three rotational velocities ($\mit\omega/\omega_{\text {crit}}$ = 0, $\mit\omega/\omega_{\text {crit}}$ = 0.50, and $\mit\omega/\omega_{\text {crit}}$ = 0.75). We find that rapid rotation leads to an expansion of the subsurface CZ, increases convective velocities, and promotes the development of this zone. Additionally, subsurface CZs can also emerge in stars with lower metallicities. Comparing our models with observations of massive stars in the Galaxy, the Large Magellanic Cloud, and the Small Magellanic Cloud, we find that rotating models better encompass the observed samples. Rotation significantly influences the evolution of the subsurface CZ in massive stars. By comparing with the observed microturbulence on the surfaces of OB stars, we propose that the subsurface CZs may be one of the sources of microturbulence.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

